Visual Grounding Helps Learn Word Meanings in Low-Data Regimes

Modern neural language models (LMs) are powerful tools for modeling human sentence production and comprehension, and their internal representations are remarkably well-aligned with representations of language in the human brain. But to achieve these results, LMs must be trained in distinctly un-human-like ways - requiring orders of magnitude more language data than children receive during development, and without perceptual or social context. Do models trained more naturalistically -- with grounded supervision -- exhibit more humanlike language learning? We investigate this question in the context of word learning, a key sub-task in language acquisition. We train a diverse set of LM architectures, with and without auxiliary visual supervision, on datasets of varying scales. We then evaluate these models' learning of syntactic categories, lexical relations, semantic features, word similarity, and alignment with human neural representations. We find that visual supervision can indeed improve the efficiency of word learning. However, these improvements are limited: they are present almost exclusively in the low-data regime, and sometimes canceled out by the inclusion of rich distributional signals from text. The information conveyed by text and images is not redundant -- models mainly driven by visual information yield qualitatively different from those mainly driven by word co-occurrences. However, our results suggest that current multimodal modeling approaches fail to effectively leverage visual information to build human-like word representations from human-scale data.

==> sections/__unused.tex <==
\subsection{Visual information provides more help to learn concrete words than abstract words.}\label{sec_res_concrete}
The benchmark results illustrate that Visual + Word models diverge from Language-Only models; however, the manner in which this difference manifests on a per-word basis remains unclear.
To better understand this difference, we explore what characteristics of words influence how well they are learned by these models.

Since the word-relatedness benchmark is where Visual + Word models achieve the most competitive results compared to Language-Only models, we first focus on how different the learned representations of grounded and ungrounded models are on this benchmark.
To be more specific, the word-relatedness judgements are computed and then cross-correlated for the Visual + Word (CLIP), the Visual + Language (GIT), and the Language-Only models trained with 2.1M image-caption pairs (50M tokens in the captions)
Although these three models achieve comparable performance, we find that their judgements are not all identical.
In fact, the correlation between the Visual + Word (CLIP) and the Language-Only models is only 0.70, which is significantly lower than their self-correlation values across different seeds (0.96 for the Language-Only model and 0.92 for the CLIP model).
The Visual + Language (GIT) model, however, yields almost the same word-relatedness judgements as the Language-Only model, as the correlation between these two models is 0.95, which is close to their self-correlation values (both 0.96).
This result not only shows that visual information can yield a totally different and still useful representation, but also suggests that the learning in GIT is dominated by cross-word distributional information when available.

We then analyze the learned representations on a per-word basis.
As the word-relatedness benchmark computes the Spearman correlation between a model and human judgements, we calculate two rank values for each pair of words, where one is from sorting all pairs by the model judgement and the other is from sorting all pairs by human judgements.
The absolute difference between these two ranks is used to approximate how human-like one pair of words is represented by the model.
To normalize this human-likeness measure, all pairs of words are further sorted from less human-like (larger absolute difference) to more human-like (smaller absolute difference) to get a ``rank in human-likeness'' measure for each pair of words, where a larger value means more human-like.
Treating this measure as the dependent variable, we run linear regressions using different features of words as independent variables, including concreteness, age of acquisition, Zipf lexical frequency, and prevalence. 
Among these features, we find that the concreteness value does not only best predict the rank in human-likeness for the Visual + Word (CLIP) model, but also clearly differentiate the grounded and ungrounded models, as it is uncorrelated with the rank measure from the language-only model (see Fig.~\ref{fig_analysis}\textbf{A} and Appendix for results of other features).
This result shows that one clear difference between Visual + Word and Language-Only models is that grounded learning better relate concrete words than abstract words.

Next, we investigate whether Visual + Word and Language-Only models differently relate nouns, verbs, and adjectives.
The dataset used in the word-relatedness benchmark contains mostly nouns~\citep{MTest3000} and some adjectives (mostly words of colors).
Therefore, we run the word-relatedness benchmark on another human judgement datasets focusing exclusively on verbs (SimVerb-3500~\citep{SimVerb3500}) and find that Visual + Word models become significantly worse than Language-Only models (see the left panel of Fig.~\ref{fig_analysis}\textbf{B}).
This is likely because image features from an unsupervised learning algorithm trained only on static images may contain very limited information for actions, which are better represented by dynamics in videos.
In addition to verbs, we also find that the color words are differently related by visual models compared to human judgements (see the right panel of Fig.~\ref{fig_analysis}\textbf{B}).
One potential explanation is that the human annotators view these color words as instances of a high-level word category, while Visual + Word models are over-dominated by the visual differences of color words.
To confirm that these results are robust to the choice of word-relatedness datasets, we re-evaluate all models on SimLex-999 and find very similar results (see Appendix Fig.~\ref{ap_fig_simlex}).
Taking together, these two additional word-relatedness results illustrate that even for this benchmark, learning only from static-image visual information is insufficient to capture the full picture of human relatedness judgements.
%Other visual information like videos and cross-word distributional information are likely needed to augment visual models.

Finally, we extend our analysis to the semantic-feature prediction benchmark.
%Going beyond the word-relatedness benchmark, we also analyze whether this concreteness feature influences the performance of the semantic-feature prediction benchmark.
%The visual and language-only models trained with 640K image-caption pairs (15M tokens in captions) are used in this analysis, as their accuracy on this benchmark is very close.
%To compare these two models, we compute the accuracy difference between them for each word and find that the concreteness feature also positively correlate with this difference (see Fig.~\ref{fig_analysis}\textbf{C}).
Similarly as the word-relatedness benchmark, we also find that Visual + Word models predict the features of concrete words more accurately than Language-Only models (see Appendix for details).
This means that visual information indeed helps better learn concrete words than abstract words.



%Coupled visual and language data are also ubiquitous on the Internet, yielding multiple high-quality and large-quantity datasets~\citep{CC12M, LAION5B, desai2021redcaps}.
%In order to model these coupled vision and language data, researchers have proposed numerous multi-modality learning algorithms connecting representations from different modalities~\citep{CLIP, GIT, Flamingo, FLAVA, unified_io}.
%However, some of these algorithms only evaluate their models on vision-language tasks, which prevents a fair comparison between these models and models only trained with language~\citep{GIT, Flamingo}.
%Other algorithms focus more on aiding visual learning using language input~\citep{CLIP}.
%Although an earlier work has claimed that multi-modality models seem to underperform their language-only counterparts on language understanding tasks~\citep{yun2021does}, that work used multi-modality learning algorithm that are outdated now (VideoBERT~\citep{sun2019videobert} and VisualBERT~\citep{li2020does}).


%The representations from grounded learning also underperform those from language-only learning in predicting lexical relations between pairs of words and identifying the Part-Of-Speech tagging of words.
%We additionally find that the architecture of fusing vision and language significantly influences the word-learning efficiency.
%Contrastive vision-language learning (CLIP~\citep{CLIP}) yields the highest efficiency when learning only from noisy image-word pairs but not from image-caption pairs, showing a surprising under-leverage of distributional information.
%Causal language modeling with abstract features of images (GIT~\citep{GIT}) leads to a less efficient word-learning and a stronger preference on distributional information when such information is provided.



\textbf{Evaluating word learning.}
Comparing the learning efficiency between models and humans requires measuring their learning abilities on the same benchmark.
However, it is challenging to directly ask models whether they can understand or produce words correctly, as is typically done in studies of child word learning \citep{CDI, WordBank}.
Recording ``attention'' patterns to visual stimuli is also implausible for language-only models, which prevents a fair comparison between grounded and ungrounded models.
Therefore, we approximate this word-learning-efficiency measure using the data efficiency on various benchmarks that evaluate how well models understand words from different aspects.
As described by \cite{miller1999knowing}, knowing the interrelations between words is critical to mastering different words.
We use two benchmarks to characterize these interrelations: word similarity and lexical relation prediction benchmarks.
Word similarity benchmarks, such as WordSim-353~\citep{WordSim353}, SimLex-999~\citep{Simlex999}, SimVerb-3500~\citep{SimVerb3500}, and MEN~\citep{MTest3000}, assess how well models capture semantic similarities between a pair of words.
Lexical relation prediction benchmarks like CogALex-V~\citep{CogALexV}, ROOT09~\citep{ROOT09}, and BLESS~\citep{BLESS} focus on how accurate models can predict nuanced relations (synonym, hyponym, etc.) between words.
Understanding a word also entails more basic aspects of its meaning: such as the fact that \emph{apples} are edible or \emph{elephants} are large.
In LMs, this can be assessed using semantic norm prediction tasks~\citep{McRae2005, Buchanan2019, chronis2023method}.
Beyond word-level representations, the ``contexts in which a word can be used to express a particular meaning are a critical component of word knowledge'' \citep{miller1999knowing}.
Our experiments assess this knowledge via part-of-speech classification and cloze completion tasks.

%Therefore, we build a new benchmark testing the abilities of models to detect unusual or incorrect contexts around one word.
%We further introduce a brain-response prediction benchmark to evaluate how similar models and humans represent sentences.
%To summarize, we test models on four word- and two context-representation benchmarks.




The first benchmark evaluates whether models can identify typical contexts in which words should appear.
%This benchmark is created by minimally changing an example sentence for one target word to make the context unusual or incorrect for this word but still grammatical.
To create this benchmark, we first select real sentences containing each target word \jda{from what corpus}, then minimally modify these sentences so that they are not longer appropriate environments for the target word. \jda{brief description of how we use big pre-trained LMs to do this modification}
For example, if we have a target word \emph{shoes} occurring in a sentence \emph{Wear your shoes}, we might alter the containing sentence to read \emph{Eat your shoes}, a significantly lower-probability environment for the target word.
%We also select this change to make the new sentence more appropriate for a distractor word.
%For instance, the example sentence ``You gotta walk away now.'' with ``walk'' as the target word is modified to ``You gotta walk \textbf{lyrics} now'' if the distractor word is ``write.''
%This new sentence is clearly incorrect. But if the word ``walk'' is replaced by ``write'', the new sentence becomes reasonable.
%Models are then evaluated by computing their surprisals on these two sentences to check if the surprisal of the original sentence is lower.
By repeating this process, we obtain
\jda{give a precise number} sentence pairs for nouns, verbs, and adjectives, yielding three sub-benchmarks shown in Fig.~\ref{fig_dist_grd_ctx_nrl}\textbf{A}.
To evaluate models on these benchmarks, we measure fraction of sentence pairs in which they assign higher probability to the original sentence compared to the modified one.




\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth] {supp_figures/iclr2024_supp_word_of_interest.pdf}
\captionof{figure}{
The word-of-interest constraint added to the Visual + Word (CLIP) models does not influence the results.
Results of Visual + Language (CLIP) and Language-Only models trained with the word-of-interest constraint are also shown here, where the captions are rewritten to keep only the words that are tested in the word-learning benchmarks.
}
\label{ap_fig_woi}
\end{figure*}


\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth] {supp_figures/which_vis_git.pdf}
\captionof{figure}{
\textbf{Changing visual encoders leads to small influence on word-learning efficiency for Visual + Word model (GIT).} Two models with different random seeds are trained in each condition. 
}
\label{ap_fig_which_vis}
\end{figure*}





\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth] {figures/dist_grd_only_bck_v4.pdf}
\vspace{-1.5em}
\captionof{figure}{
\textbf{Adding more context to Visual + Word models, or changing the model to Flamingo, offers little benefit.}
%  and can even be detrimental
The top row shows examples of small-context labels generated from the example caption in Fig.~\ref{fig_main}.
%\textbf{A} to \textbf{C}:  Performance of visual models trained with separate words (\textbf{A}), small contexts around these words (\textbf{B}), and the whole captions (\textbf{C}) as labels for images.
%\textbf{D.} Performance of visual models trained with small contexts or full captions as image labels on the context-based word-understanding benchmark. 
%\textbf{E.} Brain-response fitting results for visual models trained with full captions.
Two models with different random seeds are trained in each condition.
}
\label{fig_dist_grd_bck}
\end{figure*}

\subsection{Narrower textual contexts in grounded models yield limited benefit.}

Visual + Word and Visual + Language represent two extreme conditions about how much distributional information is included.
To explore the role of intermediate forms of distributional information, we augment visual information with some, but not all, context around the words of interest (see the top part of Fig.~\ref{fig_dist_grd_bck}).
This leads to Visual + Context models and their ungrounded counterparts, Context-Only models.
After testing these new models, we find that CLIP and GIT still fail to combine visual and distributional information to outperform Language-Only models.
%Both Visual + Context (CLIP) and Visual + Context (GIT) models are better than Context-Only models, meaning these algorithms successfully leverage visual information to supplement the cross-word distributional information contained in small contexts.
CLIP continues to illustrate a negative influence from incorporating more context (see Fig.~\ref{fig_dist_grd_bck}). 
Visual + Context (GIT) models only outperform Context-Only models on small dataset scales.
These results underscore the fact that new multi-modal models are needed to integrate both information sources effectively.


\subsection{Flamingo achieves worse results than CLIP and GIT.}
% (Since the Flamingo's results on brain-response prediction is quite eye-catching, it's a bit weird to introduce this after the context benchmarks)
To further evaluate the robustness of these results to choices of model architecture, we repeat a subset of our analysis 
in Flamingo models~\citep{Flamingo}.
This model architecture first extracts a summary vector from the image features and then modulates language representations using this vector through a cross-attention mechanism (see Appendix ~\ref{ap_flamingo} for details).
%The original Flamingo algorithm loads pretrained weights for the transformer layers only processing texts and freezes these weights.
%Since we explore how visual information helps learning, we initialize the text transformer from scratch and optimize it as well as the Perceiver Resampler and the cross-attention layers to predict next words using their prior context.

%After training and evaluating Flamingo models, 
We find that these models underperform CLIP and GIT in leveraging visual information.
On all benchmarks except the POS benchmark, Flamingo models perform no better than Language-Only models.
Flamingo models also fail to benefit from more context than what is used in Visual + Context models. 
%indicating that this algorithm learns more from the local context of words.
This might be why Visual + Language (Flamingo) models are more efficient learning in the POS benchmark, as Context-Only models also show similarly higher efficiency on this benchmark.
To confirm that this result is robust, we vary an important hyperparameter in Flamingo but find it barely influences the performance (see Appendix Fig.~\ref{ap_fig_flmg_var}).  



To further explore the role of distributional information in learning, we include more context to single-word labels, yielding Visual + Context and Context-Only models (see Appendix~\ref{ap_context}).
The results of these limited-context models again confirm the interference between visual and linguistic distributional information in learning (see Appendix Fig.~\ref{fig_dist_grd_bck}).
We also test Flamingo~\cite{Flamingo} and find it underperforms CLIP and GIT (see Appendix Fig.~\ref{fig_dist_grd_bck}).
This indicates that how Flamingo fuses visual and language information, which is through cross-modality attentions from vision to text, is less efficient in learning word meanings than the fusing mechanisms of CLIP and GIT.
